A Physics-Informed Digital Twin Framework for Calibrated Sim-to-Real FMCW Radar Occupancy Estimation

Learning robust radar perception models directly from real measurements is costly due to the need for controlled experiments, repeated calibration, and extensive annotation. This paper proposes a lightweight simulation-to-real (sim2real) framework that enables reliable Frequency Modulated Continuous Wave (FMCW) radar occupancy detection and people counting using only a physics-informed geometric simulator and a small unlabeled real calibration set. We introduce calibrated domain randomization (CDR) to align the global noise-floor statistics of simulated range-Doppler (RD) maps with those observed in real environments while preserving discriminative micro-Doppler structure. Across real-world evaluations, ResNet18 models trained purely on CDR-adjusted simulation achieve 97 percent accuracy for occupancy detection and 72 percent accuracy for people counting, outperforming ray-tracing baseline simulation and conventional random domain randomization baselines.

==> sec/related_work.tex <==
\section{Related Work}
\label{sec:related_work}
\textcolor{red}{NEED CITATIONS}
\paragraph{Radar-based occupancy and people counting with sim2real.}
FMCW radar has been widely explored for human detection, tracking, and activity recognition in indoor environments due to its robustness to lighting and privacy advantages. Prior approaches often rely on handcrafted features from RD or range--angle maps, or on convolutional neural networks trained on curated real datasets.
However, most datasets are limited to a handful of environments, sensor placements, and subject populations, resulting in models that are brittle when deployed elsewhere.

\paragraph{Digital twins and radar simulation.}
Electromagnetic solvers and ray-tracing-based radar simulators enable realistic modeling of multipath, materials, and motion, opening the possibility of training models entirely in simulation. In camera-based perception, several works have successfully adopted digital twins for autonomous driving and robotics. For radar, research has begun to explore synthetic RD maps for automotive and indoor sensing, but sim-to-real gaps in noise, clutter, and sidelobe structure remain a major challenge.

\paragraph{Domain randomization and sim-to-real transfer.}
Domain randomization (DR) is a standard strategy to bridge simulation and reality: during training, synthetic observations are heavily randomized so that real data appear as a special case of the synthetic distribution. Variants include appearance randomization, physics or sensor parameter randomization, and style transfer using generative models. In radar, DR has been applied by perturbing noise floors, clutter levels, or signal parameters. Uncalibrated DR, however, may either under-compensate (leaving a residual gap) or over-randomize (destroying informative structure), requiring extensive hyperparameter tuning.

\paragraph{Calibration with unlabeled real data.}
A complementary strategy is to use small amounts of unlabeled real data to calibrate synthetic data generation or normalization, e.g., matching feature distributions or aligning summary statistics. The present work falls into this category, proposing a particularly simple form of calibration: learning the global noise-floor distribution from real RD maps and using it to bound simulated noise. This preserves simulated human signatures while aligning background statistics and requires no labels, adversarial training, or complex architectures.





 
\begin{figure*}[!t] % top of next page is typical/allowed for IEEEtran
% \begin{figure}[htb] % top of next page is typical/allowed for IEEEtran
  \centering    \includegraphics[
    width=\textwidth,
    height=.38\textheight,   % shrink vertically
    keepaspectratio,         % never distort
  ]{figures/Digital_twin_plot_2.pdf}
  \caption{\textcolor{red}{TODO}}
  \label{fig:Digital_twin_plot}
\end{figure*}



% \begin{figure*}[!t] % top of next page is typical/allowed for IEEEtran
%   \centering    \includegraphics[
%     width=\textwidth,
%     height=.28\textheight,   % shrink vertically
%     keepaspectratio,         % never distort
%   ]{figures/feature_maps_grid_2.png}
%   \caption{\textcolor{red}{TODO}}
%   \label{fig:Digital_twin_plot}
% \end{figure*}
% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.25]{figures/feature_maps_grid_2.png}
%     \caption{Example figure for \textit{Journal of Computational Vision and Imaging Systems}.}
%     \label{fig1}
% \end{figure}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/feature_maps_grid_pub.pdf}
    \caption{
    Qualitative comparison of early feature maps for simulated and real radar range-Doppler inputs.
    (a,d) inputs;
    (b,e) features from the Naive model trained only on unmodified simulation;
    (c,f) features from the CDR-trained model.
    CDR preserves discriminative micro-Doppler patterns on real measurements while suppressing background artifacts, indicating improved domain alignment.
    }
    \label{fig:feature_maps}
\end{figure}




\begin{figure*}[!t] % top of next page is typical/allowed for IEEEtran
% \begin{figure}[htb] % top of next page is typical/allowed for IEEEtran
  \centering    \includegraphics[width=0.8\textwidth, 
      trim=0pt 170pt 0pt 35pt, 
      clip
  % scale=0.27
    % width=\textwidth,
    % height=\textheight,   % shrink vertically
    % keepaspectratio,         % never distort
  ]{figures/CDR_flowchart.pdf}
  \caption{\textcolor{red}{TODO}}
  \label{fig:Digital_twin_plot}
\end{figure*}



\begin{figure}[htb] % top of next page is typical/allowed for IEEEtran
  \centering    \includegraphics[scale=0.36]{figures/cdr_statistical_alignment.pdf}
  \caption{\textcolor{red}{TODO}}
  \label{fig:Digital_twin_plot}
\end{figure}

\begin{figure*}[!t]
  \centering    \includegraphics[
    width=\textwidth,
    height=.3\textheight,   % shrink vertically
    keepaspectratio,         % never distort
  ]{figures/training_curves_naive_random_cdr.pdf}
  \caption{\textcolor{red}{TODO}}
  \label{fig:Digital_twin_plot}
\end{figure*}
% All figures must include a figure number as well as an associated caption. An example figure is shown in Fig.~\ref{fig1}.

% \begin{figure}[t]
%     \centering
%     \includegraphics[scale=0.7]{JCVIS}
%     \caption{Example figure for \textit{Journal of Computational Vision and Imaging Systems}.}
%     \label{fig1}
% \end{figure}

